Discovery of a disrupting open cluster far into the Milky Way halo: a recent star formation event in the leading arm of the Magellanic stream?

We report the discovery of a young (${\rm age} \sim 130~{\rm Myr}$), low-mass ($M \sim 1200~{\rm M}_\odot$), metal-poor ($[{\rm Fe}/{\rm H}] \sim -1.1$) stellar association at a heliocentric distance $D \approx 29~{\rm kpc}$, placing it far into the Milky Way halo. At its present Galactocentric position $(R, z) \sim (23, 15)~{\rm kpc}$, the association is (on the sky) near the leading arm of the gas stream emanating from the Magellanic cloud system, but is located $\approx 60^\circ$ from the Large Magellanic Cloud (LMC) center on the other side of the Milky Way disk. If we assume that the cluster is co-located with HI gas in the stream, we directly measure the distance to the leading arm of the Magellanic stream. The measured distance is inconsistent with stream predictions from models of the LMC/SMC interaction and infall into the Milky Way that do not account for ram pressure and gas interaction with Milky Way disk. The estimated age of the cluster is consistent with the time of last passage of the leading arm gas through the Galactic midplane, and we therefore speculate that this star-formation event was triggered by its the last disk midplane passage. Most details of this idea remain a puzzle: the Magellanic stream has low column density, the Milky Way disk at this large radius has low gas density, and the relative velocity of the leading arm gas and Milky Way gas is large. However it formed, the discovery of a young stellar cluster in the Milky Way halo presents an interesting opportunity for study. This cluster was discovered with Gaia astrometry and photometry alone, but folow-up DECam photometry was crucial for measuring its properties.

==> Makefile <==
LATEX       = pdflatex -interaction=nonstopmode -halt-on-error
BASH        = bash -c
ECHO        = echo
RM          = rm -rf
TMP_SUFFS   = pdf aux bbl blg log dvi ps eps out brf
CHECK_RERUN =
GIT_PATH    = .git/

NAME = ms

all: ${NAME}.pdf

${NAME}.pdf: ${NAME}.tex ms.bib
	${LATEX} ${NAME}
	bibtex ${NAME}
	${LATEX} ${NAME}
	( grep "Rerun to get" ${NAME}.log && ${LATEX} ${NAME} ) || echo "Done."
	( grep "Rerun to get" ${NAME}.log && ${LATEX} ${NAME} ) || echo "Done."


clean:
	${RM} $(foreach suff, ${TMP_SUFFS}, ${NAME}.${suff})
	${RM} *.aux
	${RM} *Notes.bib

submit: ${NAME}.pdf
	make
	tar -czvf archive.tar.gz $$(git ls-tree --name-only HEAD | grep -v ".gitignore\|Makefile\|figures") -C ./figures/ $$(cd figures && git ls-files)
	echo "archive.tar.gz created"

